The First OpenFOAM HPC Challenge (OHC-1)

The first OpenFOAM HPC Challenge (OHC-1) was organised by the OpenFOAM HPC Technical Committee (HPCTC) to collect a snapshot of OpenFOAM's computational performance on contemporary production hardware and to compare hardware-constrained submissions with software-track optimisations. Participants ran a common incompressible steady-state RANS case, the open-closed cooling DrivAer (occDrivAer) configuration, on prescribed meshes, submitting either with the reference setup (hardware track) or with modified solvers, decomposition strategies, or accelerator offloading (software track). In total, 237 valid datapoints were submitted by 12 contributors: 175 in the hardware track and 62 in the software track. The hardware track covered 25 distinct CPU models across AMD, Intel, and ARM families, with runs spanning from single-node configurations up to 256 nodes (32768 CPU cores). Wall-clock times ranged from 7.8 minutes to 65.7 hours and reported energy-to-solution from 2.1 to 236.9 kWh. Analysis of the hardware track identified a Pareto front of optimal balance between time- and energy-to-solution, and revealed that on-package high-bandwidth memory (HBM) dominates single-node performance for next-generation CPUs. Software-track submissions achieved up to 28% lower energy per iteration, 17% higher maximum performance per node, and 72% shorter minimum time per iteration than the best hardware-track results, with full GPU ports and selective-memory optimisations leading the performance range. This manuscript describes the challenge organisation, the case setup and metrics, and presents the main findings from both tracks together with an outlook for future challenges.

==> parts_refactored/conclusion_broken.tex <==
\section{Conclusion and Outlook} \label{sec:conclusion}

The first OpenFOAM HPC Challenge (OHC-1) collected 237 valid datapoints from 12
contributing organisations across a hardware track (175 submissions) and a
software track (62 submissions). Participants ran the common occDrivAer
steady-state RANS case on prescribed meshes, with hardware-track runs restricted
to the reference setup and software-track runs allowing approved solver and
decomposition modifications.

\subsection{Hardware-track findings}

The hardware track provided a diverse baseline of \OF performance on current
production systems, covering 25 CPU models from AMD, Intel, and ARM, with runs
from single-node configurations up to 256 nodes. The key findings are:
\begin{itemize}
\item A Pareto front of optimal balance between time-to-solution and
  energy-to-solution was identified, highlighting that increasing parallelism
  yields diminishing time savings at substantially higher energy cost.
\item At small scale, next-generation CPUs (ARM, Intel, AMD) with on-package
  high-bandwidth memory (HBM) and many-core architectures show significantly
  improved single-node performance.
\item At large scale, inter-node communication dominates performance. Many-core
  architectures pose a particular challenge for \OF, which currently relies solely
  on MPI parallelism. A practical strong-scaling limit of approximately
  10\,000~cells per core was observed.
\item The maximum reported hardware-track performance was approximately
  630~MFVOPS per node, with a minimum energy per iteration of about 2613\,J.
\end{itemize}

\subsection{Software-track findings}

The software track demonstrated that substantial gains are achievable through
algorithmic and implementation optimisations. Software-track submissions addressed
multiple optimisation areas---full GPU ports, GPU linear-solver offloading,
decomposition optimisation, mixed precision, selective memory allocation, and
coherent I/O---and achieved:
\begin{itemize}
\item up to 28\% lower minimum energy per iteration (1867 \,J vs.\ 2613\,J);
\item 17\% higher maximum FVOPS per node (737 vs.\ 629~MFVOPS);
\item  A reduction of up to 720\% required to compute a single timeshorter step.minimum time per iteration (0.11\,s vs.\ 0.37\,s).
\end{itemize}
A key insight is that software optimisations on older-generation hardware can
outperform unoptimised runs on newer-generation CPUs, underscoring the importance
of co-optimising algorithms alongside hardware.

\subsection{Outlook}

OHC-1 establishes a reference dataset and unified metrics (FVOPS, energy per
iteration, time-to-solution) for future comparisons. Contributions exceeded
expectations, but the submission format needs to be tightened for future editions
to further improve comparability. Planned improvements for follow-up challenges
include:
\begin{itemize}
%\item extending the challenge to additional cases and mesh sizes;
\item encouraging more software-track participation (currently $\sim$20\% of
  total submissions);
\item systematic investigation of network interconnect effects;
\item deriving best-practice guidelines based on the collected submissions;
\item promoting the occDrivAer case as a more relevant community benchmark than
  the commonly used Lid-Driven Cavity;
\item continued publication and curation of the results dataset to enable
  further community analysis (see \Cref{sec:repository}).
\end{itemize}
The HPCTC
repository\footnote{\url{https://develop.openfoam.com/committees/hpc}} remains
the central place for case setups and submission guidelines. All OHC-1
submission data, analysis notebooks, and presentations are publicly available in
the OHC-1 data repository~\cite{ohc1_repo} as described in
\Cref{sec:repository}.


==> parts_refactored/hardwaretrack_broken.tex <==
\subsection{Hardware Track} \label{sec:hardware_track} \label{sec:res_hardware_track}

Hardware-track submissions used the reference case and an official \OF release, whereby only hardware, node count, and system software could vary.
In total, 175 data points were submitted., where \cref{fig:overview_hardware_track} gives an overview of the submissions, showing the reported time-to-solution over a broad set of employed CPUs and the different mesh sizes. As shown in \cref{fig:overview_mesh_heatmap} all three mesh sizes had numerous submissions, with some participants, e.g.\ ~5, 7, and 13 submitting an equal amount of data points for all meshes. Some participants had a stronger focus on either coarse or fine mesh investigations, e.g.\ ~participants 8 and 6. In total, most data points where submitted for the coarse mesh and the least number for the medium, likely because participants either focused on the single node performance or the extreme scaling results. Furthermore the submitted data in the hardware track covers 20 distinct CPU models across three major vendor families: AMD (81 submissions), ARM~(34), and Intel~(60). \Cref{fig:overview_hardware_cpu} shows a breakdown of the number of  submissions into CPU vendors and individual CPU generations.
\begin{figure}
     \centering
     \begin{subfigure}[b][5cm][]{0.30\textwidth}
         \centering
        \includegraphics[height=5cm]{figures/submissions_overview_aspect.png}
        \caption{\label{fig:overview_hardware}}
     \end{subfigure}
           \hfill
     \begin{subfigure}[b][5cm][]{0.14\textwidth}
         \centering
         \includegraphics[height=5cm]{figures/submissions_heatmap.png}
                  \caption{\label{fig:overview_mesh_heatmap}}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b][5cm][]{0.50\textwidth}
         \centering
\includegraphics[height=5cm]{figures/submissions_overview_cpu.png}             \caption{\label{fig:overview_hardware_cpu}}
     \end{subfigure}
    \caption{Overview of hardware-track submissions, (a) Time-to-solution over number of utilized CPU cores, (b) number of submissions based on mesh type and contributor ID, (c) number of submissions based on CPU vendor and CPU Generation.\label{fig:overview_hardware_track}}
\end{figure}

\subsubsection{Energy--time trade-off and Pareto front}

A central question in HPC workloads is the trade-off between time-to-solution (TTS) and energy-to-solution (ETS).
\Cref{fig:TTS_ETS_MESH_singleNode} presents such a trade-offshows
energy-to-solution versus wall-clock time for all hardware-track runs, faceted by mesh size. Pareto fronts are shown as black lines indicating the optimal balance between TTS and ETS achieved with hardware released prior to that year.  From the pareto fronts, t
Three distinct operating regimes are visible:
\begin{enumerate}
\item \emph{EMost efficient}: runs that minimise energy consumption at the cost of
  longer execution times (typically single-node or small-scale runs on
  energy-efficient hardware).
\item \emph{Fastest}: runs that minimise wall-clock time by using many nodes, at
  the expense of higher total energy.
\item \emph{BGood balance}: runs that achieve a practical compromise between
  energy and time.
\end{enumerate}
%
%A Pareto front of non-dominated solutions, for which no other submission
%achieves simultaneously lower energy \emph{and} lower time, was identified for
%each mesh.
The shapes of the Pareto fronts for lower values of consumed energy demonstrate that relatively large improvements (lower values) of TTS can be achieved with low increases in ETS.
On the other hand, for high ETS
The shape of the Pareto front confirms that increasing parallelism yields diminishing time savings while incurring substantially higher energy costs, consistent with strong-scaling saturation effects discussed below.
\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.95\textwidth]{figures/TTS_ETS_facetGrid_pareto_year.png}
  \caption{Energy-to-solution vs.\ time-to-solution for hardware-track runs,
    faceted by mesh size. Operating regimes and the Pareto front of optimal
    energy--time balance are indicated.}
  \label{fig:TTS_ETS_MESH_singleNode}
\end{figure}
\iffalse
\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.95\textwidth]{figures/TTS_ETS_facetGrid-singleNode.png}
  \caption{Energy-to-solution vs.\ time-to-solution for hardware-track runs,
    faceted by mesh size. Operating regimes and the Pareto front of optimal
    energy--time balance are indicated.}
  \label{fig:TTS_ETS_MESH_singleNode}
\end{figure}
\fi
%\Cref{fig:TTS_ETS_cpufamily} provides a complementary view of the same 
energy--time trade-off, with points coloured by CPU vendor family (AMD, Intel, 
ARM). 
For each mesh, the three families occupy overlapping but distinct regions of
the plot. ARM submissions tend to cluster in the lower-energy region, reflecting
recent many-core, high-bandwidth-memory designs. AMD and Intel submissions span a
wider range of node counts and correspondingly wider ranges of both time and
energy. Across all three meshes, the same qualitative trend holds: runs using
more nodes reduce time-to-solution but shift upward and to the right in energy
consumption.
\iffalse
\begin{figure*}[!ht]
  \centering
  \includegraphics[width=0.95\textwidth]{figures/TTS_ETS_facetGrid_cpufamily.png}
  \caption{Time-to-solution vs.\ energy-to-solution for all hardware-track runs,
    faceted by mesh size and coloured by CPU vendor family.}
  \label{fig:TTS_ETS_cpufamily}
\end{figure*}
\fi
\subsubsection{Strong-scaling behaviour}\label{sec:hw_scaling}

Strong scaling, which represents ---running a fixed problem size on an increasing number of 
cores, ---reveals two distinct performance-limiting regimes:
\begin{itemize}
\item \emph{Single-node scaling limit:} Within a single node, performance is
  bounded by memory bandwidth.  As the number of cores per node increases,
  contention for shared memory buses limits the per-core throughput. This effect
  is especially pronounced for many-core architectures.
\item \emph{Multi-node scaling limit:} Beyond a single node, inter-node
  communication dominates the execution time. Since \OF relies exclusively on MPI
  for parallelism, the communication overhead grows with the surface-to-volume
  ratio of the domain decomposition. A practical scalability limit of
  approximately 10\,000~cells per core was observed across submissions. Below
  this threshold, communication costs exceed computational work. Depending on the CPU architecture, this limit may be larger.
\end{itemize}

\Cref{fig:strong_scaling} shows strong-scaling behaviour across three mesh resolutions (coarse, medium, fine), three CPU families (AMD, ARM, Intel), and processor generations within each family.
Time-to-solution is plotted against core count, with the corresponding cells-per-core indicated along the top axis.
The data is represented by means of a scatter plot with the associated curves that are fitted using local regression.
Only data with more than two points per mesh and CPU generation is included in the plot to enable meaningful fitting.
Across all architectures and mesh sizes, time-to-solution decreases with increasing core count, confirming expected strong scaling behaviour.
However, none of the configurations exhibit ideal linear scaling over the full range.
In some cases, the slope of the curves decreases at higher core counts, indicating reduced parallel efficiency as the workload per core diminishes and communication overhead becomes more significant.
The relevant cells-per-core ratio is about 10000.
Within each CPU family, newer generations generally achieve lower absolute runtimes at comparable core counts.


\begin{figure*}[!ht]
  \centering
  %\includegraphics[width=0.95\textwidth]{figures/strong_scaling_combined.png}
  % \includegraphics[width=0.95\textwidth]{figures/TTS_Cores_facetGrid_alt.png}
  \includegraphics[width=\textwidth]{figures/TTS_cores_facetGrid_mesh_CPUVendor.png}
  \caption{
  Strong scaling: time-to-solution vs.\ number of CPU cores for the coarse (top), medium (centre), and fine (bottom) meshes with a segmentation based on CPU family: AMD (right), ARM (.
  Lines connect data points from the same CPU sub-model, coloured by vendor family and styled by CPU generation.}
  \label{fig:strong_scaling}
\end{figure*}

\subsubsection{Parallel efficiency}\label{sec:hw_parallel_eff}

To quantify how effectively additional cores reduce time-to-solution, we compute a normalised parallel efficiency metric.
For each CPU generation with multi-node data, the efficiency is defined as the ratio of the minimum core-weighted time (i.e.\ the most efficient single run) per mesh to the core-weighted time of each run:
\begin{equation}
  \eta = \frac{\min_{i}(T_i \cdot N_i)}{T \cdot N}\,,
  \label{eq:parallel_eff}
\end{equation}
where $T$ is the time-to-solution, $N$ is the number of CPU cores, and the minimum is taken over all multi-node runs for the mesh.

\Cref{fig:parallel_efficiency} shows the parallel efficiency for the three mesh sizes.
Efficiency drops below unity as the core count increases, indicating communication overhead.
The rate of decline depends on CPU generation and vendor family: architectures with higher per-core memory bandwidth and more capable interconnects maintain higher efficiency at larger core counts.
Some of the CPU generations demonstrate higher parallel efficiency with the increasing number of cores indicating super-linear scaling, which is a known pattern for modern computer architectures~\cite{Galeazzo2024a}.
% For the coarse mesh, efficiency falls below 50\% at approximately 10\,000--20\,000 cores, consistent with the scalability limit discussed above.

\begin{figure*}[!ht]
  \centering
  \includegraphics[width=\textwidth]{figures/efficiency_cores_facetGrid_mesh_CPUVendor.png}
  \caption{Parallel efficiency vs.\ number of CPU cores for the coarse (left)
    and medium (right) meshes. Coloured by vendor family, styled by CPU
    generation. Only CPU sub-models with more than two multi-node data points are
    shown.}
  \label{fig:parallel_efficiency}
\end{figure*}

\subsubsection{Single-node performance and the HBM/LLC effect}\label{sec:hw_single_node}

To separate compute performance from interconnect effects, single-node runs were
analysed separately. These submissions show that \emph{on-package memory
dominates single-node performance}. CPUs equipped with High-Bandwidth Memory
(HBM) or large Last-Level Caches (LLC) achieve significantly higher FVOPS per
node than traditional architectures with the same core count. This is consistent
with the memory-bandwidth-bound nature of sparse iterative solvers used in \OF:
the working set of \OF's field operations and linear-algebra kernels benefits
directly from higher memory bandwidth and larger on-chip caches.

\Cref{fig:singlenode_LLC} shows the single-node energy--time trade-off with
data points coloured by last-level cache category. For the coarse and medium
meshes, submissions with larger LLC/HBM configurations consistently occupy the
lower-left (faster, more efficient) region of the plot, confirming that
on-package memory capacity is a primary determinant of single-node performance.
For the fine mesh, fewer participants were able to fit the problem on a single
node, limiting the available data; however, the available results confirm the
same trend.

\begin{figure*}[!ht]
  \centering
  \includegraphics[width=0.95\textwidth]{figures/singlenode_TTS_ETS_LLC.png}
  \caption{Single-node runs: time-to-solution vs.\ energy-to-solution, faceted
    by mesh size and coloured by last-level cache category. CPUs with
    larger on-package memory (HBM, large LLC) cluster in the lower-left
    (faster, more energy-efficient) region.}
  \label{fig:singlenode_LLC}
\end{figure*}

Overall, the hardware track established a baseline of \OF performance on current
production systems and showed clear sensitivity to CPU generation, mesh size, and
scaling across nodes. The maximum reported performance in the hardware track was
approximately 630~MFVOPS per node, with a minimum energy per iteration of about
2613\,J.

\subsubsection{Network interconnect effect}

The effect of the network interconnect on multi-node scaling is an important but
difficult factor to isolate, as it requires dedicated comparison runs on the same
CPU with different interconnects. Preliminary observations from submissions using
FDR (40\,GBit/s) and Slingshot (200\,GBit/s) interconnects suggest that higher
bandwidth and lower latency interconnects improve strong-scaling behaviour,
particularly at high core counts where communication dominates. A more systematic
study of network effects is planned for future OHC editions.


==> parts_refactored/introduction_broken.tex <==
%-----------------------------------------------------------------------
%      Start introduction here and continue with additional sections
%-----------------------------------------------------------------------

\section{Introduction}

OpenFOAM is extensively utilised in both academia and industry for research and
design, with many applications requiring large computational resources. It is
therefore common to find OpenFOAM among the principal consumers of compute capacity on
HPC clusters. To support future improvements in resource efficiency, the first
OpenFOAM HPC Challenge (OHC-1) was launched by the OpenFOAM HPC Technical
Committee (HPCTC). Challenge problems in the  broader field of high performance computing (HPC), are a commonly used tool to test hardware performance or to compare algorithmic approaches and
implementations. Well-known examples include the High Performance Linpack (HPL)
from the HPCC suite~\cite{dongarra2017hpc}, which underpins the TOP500 list, and
domain-specific challenges in areas such as automotive
CFD~\cite{autocfd2,autocfd3,autocfd4}. The term ``challenge'' is used here to
encourage community contributions aimed at improving computational efficiency
rather than only reporting baseline performance.

The goal of OHC-1 was to to gather a snapshot of \OF's performance on current production
hardware and to enable comparison of hardware configurations with software
optimisations. 
Furthermore, tThe initiative aimed to:
\begin{itemize}
\item collect data for evaluating future algorithmic and implementation choices
  in \OF;
\item assess efficiency and scalability across hardware platforms;
\item compare performance of recent \OF variants and software optimisations;
\item propose unified metrics (e.g.\ FVOPS, energy per iteration,
  time-to-solution) to guide development on next-generation systems;
\item promote a more relevant community benchmark case than the commonly used
  Lid-Driven Cavity 3D case 
\footnote{\url{https://develop.openfoam.com/committees/hpc/-/tree/develop/incompressible/icoFoam}}.
\end{itemize}
The results of 
In the broader field of high performance computing (HPC), challenge problems are
used to test hardware performance or to compare algorithmic approaches and
implementations. Well-known examples include the High Performance Linpack (HPL)
from the HPCC suite~\cite{dongarra2017hpc}, which underpins the TOP500 list, and
domain-specific challenges in areas such as automotive
CFD~\cite{autocfd2,autocfd3,autocfd4}. The term ``challenge'' is used here to
encourage community contributions aimed at improving computational efficiency
rather than only reporting baseline performance.

OHC-1 werewas presented as a mini-symposium at the 2025 OpenFOAM Workshop in Vienna
on July~1, 2025. The challenge attracted 240+ data points contributed by 12
organisations from across academia and industry, of which 237 passed validation.
The combined reported energy consumption of all submissions was approximately
4715\,kWh.

The manuscript is structured as follows. \Cref{sec:rules} describes the
organisation of the HPC Challenge and the choice of the test case. \Cref{sec:setup}
gives the case setup, mesh options, and metrics. \Cref{sec:repository} describes
the public data repository where all submissions and analysis tools are
available. \Cref{sec:analysis} summarises the submitted datapoints and
\Cref{sec:hardware_track,sec:software_track} present the main findings of the
hardware and software tracks. \Cref{sec:conclusion} concludes with a summary
and outlook for future challenges.


==> parts_refactored/organisation_broken.tex <==
%-----------------------------------------------------------------------
%      Start introduction here and continue with additional sections
%-----------------------------------------------------------------------

\section{Challenge Structure and Procedure} \label{sec:rules}

After defining the computational scope of the challenges, the procedure was structured as illustrated in \cref{fig:challenge_procedure}. Data submissions were categorized into two tracks:
\begin{description}
\item[Hardware track.] Participants used the provided case setup and an official
  \OF release. Only the hardware, number of nodes and cores, and system software
  stack could vary.
\item[Software track.] Any \OF version and custom solvers or modifications were
  allowed, provided the mesh and physical model remained unchanged and solution
  The proposed topics for investigation in the software track included accelerators, pre-/post-processing (I/O), mixed-precision arithmetic, linear solvers, and renumbering/decomposition strategies. Submissions were accepted after the validation of computational results described in section~\ref{sec:validation}.
\end{description}
The submitted results were then analyzed by the organizing committee based on a set of predefined metrics. A comprehensive analysis of the hardware track and software track results was subsequently presented by the organizers in the form of a mini-symposium. In addition, participants delivered in-depth presentations discussing their individual contributions and investigations.


% feel free to improve this figure
%https://excalidraw.com/#room=144699b8dccab23d45fa,mZdgh77eFr5mYl1foTCvGg
\begin{figure*}[!ht]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/ohc-workflow.png}
  \caption{Overview of the OHC-1 procedure}
  \label{fig:challenge_procedure}
\end{figure*}

%$\Submissions were categorised into two tracks:
\begin{description}
\item[Hardware track.] Participants used the provided case setup and an official
  \OF release. Only the hardware, number of nodes and cores, and system software
  stack could vary.
\item[Software track.] Any \OF version and custom solvers or modifications were
  allowed, provided the mesh and physical model remained unchanged and solution
  The proposed topics for investigation in the software track included accelerators, pre-/post-processing (I/O), mixed-precision arithmetic, linear solvers, and renumbering/decomposition strategies. Submissions were accepted after the computational results validation described in section~\ref{sec:validation}.
\end{description}

% feel free to improve this figure
%https://excalidraw.com/#room=144699b8dccab23d45fa,mZdgh77eFr5mYl1foTCvGg
\begin{figure*}[!ht]
  \centering
  \includegraphics[width=0.75\textwidth]{figures/hpc_challenge_flowChart.png}
  \caption{Overview of the OHC-1 procedure}
  \label{fig:meancalc_example}
\end{figure*}


\subsection{Metrics}\label{sec:metrics}

The following metrics were used to evaluate and compare the submissions in both tracks.

\begin{description}
\item[Time-to-solution (TTS)] The wall-clock time from the start of the main
  solver to completion of the prescribed number of iterations, excluding
  pre-processing and initialisation.
\item[Energy-to-solution (ETS)] The total energy consumed during the solver
  run.  Where direct power measurements were not available, energy was estimated
  from the Thermal Design Power~(TDP) of the CPUs/GPUs.
\item[Pre-processing wall-clock time] The wall-clock time for running the utilities that prepare the case for the run of the main solver application, e.g. decomposition, renumbering, initialisation with potentialFoam.
\item[Time per iteration] The mean wall-clock time of a single SIMPLE iteration.
\item[Energy per iteration] The mean energy consumed per SIMPLE iteration, derived from ETS divided by the number of iterations.
\item[FVOPS (Finite-Volume Operations Per Second)] A throughput metric proposed in~\cite{Galeazzo2024a} defined as the number of mesh cells multiplied by the number of iterations, divided by the wall-clock time:
  \begin{equation}
    \text{FVOPS} = \frac{N_\text{cells} \times N_\text{iter}}{t_\text{WC}}\,.
    \label{eq:fvops}
  \end{equation}
  FVOPS is often reported per node to enable comparison across different node counts.
\item[FVOPS per energy] The ratio of FVOPS to energy, giving an
  energy-efficiency throughput metric.
\end{description}
%\subsection{Assumptions and disclaimers}\label{sec:disclaimers}
During the data collection and analysis process, several corrections and
assumptions were necessary:
\begin{itemize}
\item The number of cores was corrected to represent \emph{physical} cores;
  hyper-threading was disregarded.
\item If not reported by the participants, some values were added based on publicly available data
  (e.g.\ TDP according to the CPU model).
\item The energy analysis is \emph{mostly based on theoretical TDP values} rather
  than direct power measurements, which introduces uncertainty.  Only a small
  number of submissions provided energy data from total cluster measurements.
\item The focus of this work lies on providing an overview of the complete data
  set; analysis of individual simulations or submissions are outside of the scope. When available references to further publications for indepth analysis is provided.%  is covered in the participants' talks presented at the OHC-1 mini-symposium.
\end{itemize}



\subsection{Submission Validation} \label{sec:validation}

Since Hardware-track submissions used the prescribed setup. Their correctness was
inherent in the use of the reference case. In contrast, Software-track submissions required
additional validation to ensure that solution quality was preserved despite any modifications in the software, case decomposition, or employed  solver
or algorithmsic modifications. Participants were required to extract force
coefficient convergence histories at run time and analyse the mean and variance of 
the aerodynamic coefficients ($C_d$, $C_l$, $C_s$) using the \texttt{meanCalc}\footnote{\url{meancalc.upstream-cfd.com/}}
utility. The validity criterion was
\begin{equation}
  2\,\sigma(\mu) < 0.0015\,,
  \label{eq:validation}
\end{equation}
where $\sigma(\mu)$ denotes the standard deviation of the running mean of the 
respective force coefficient. Reference values obtained with standard \OF on the
fine mesh were
$C_d = 0.262$,
$C_l = 0.0787$, and
$C_s = 0.0116$.
The data analysis team double-checked and cross-compared reported values with the 
submitted time series data.

\Cref{fig:meancalc_example} illustrates the validation process for an example
software-track submission (CINECA, fine mesh). The top row shows the
instantaneous force coefficients together with the running mean computed from
iteration~2000 onwards. The bottom row shows the convergence of
$2\,\sigma(\mu)$, which must fall below the threshold of~0.0015 for each
coefficient. For this submission the final values are
$2\,\sigma(\mu)_{C_d} = 2.1\times 10^{-4}$,
$2\,\sigma(\mu)_{C_l} = 9.1\times 10^{-4}$, and
$2\,\sigma(\mu)_{C_s} = 4.1\times 10^{-4}$,
all well within the acceptance criterion. The converged running-mean coefficients
($C_d = 0.2624$, $C_l = 0.0735$, $C_s = 0.0114$) are in reasonable agreement
with the reference values, confirming that the software modifications preserved
solution accuracy.

\begin{figure*}[!ht]
  \centering
  \includegraphics[width=0.95\textwidth]{figures/meancalc_validation_example.png}
  \caption{Example meanCalc validation for a software-track submission
    (CINECA, fine mesh). Top row: instantaneous force coefficients (light
    blue) with running mean from iteration~2000 (dark blue) and reference value
    (red dashed). Bottom row: convergence of $2\,\sigma(\mu)$ towards the
    acceptance threshold of~0.0015 (red dashed).}
  \label{fig:meancalc_example}
\end{figure*}

\subsection{Assumptions and disclaimers}\label{sec:disclaimers}

During the data collection and analysis process, several corrections and
assumptions were necessary:
\begin{itemize}
\item The number of cores was corrected to represent \emph{physical} cores;
  hyper-threading was disregarded.
\item If not reported, some values were added based on publicly available data
  (e.g.\ TDP according to the CPU model).
\item The energy analysis is \emph{mostly based on theoretical TDP values} rather
  than direct power measurements, which introduces uncertainty.  Only a small
  number of submissions provided energy data from total cluster measurements.
\item The focus of this paper lies on providing an overview of the complete data
  set; analysis of individual simulations or submissions is covered in the
  participants' talks presented at the OHC-1 mini-symposium.
\end{itemize}


==> parts_refactored/setup_broken.tex <==
\section{Case Setup}\label{sec:setup}\label{sec:case-setup}

The HPCTC selected a single test case that had to be representative of typical
industrial usage, computationally demanding, and suitable as a surrogate for
common simulation workloads without relying on features that would exclude
alternative implementations. Based on these criteria, the casea case with the
external aerodynamic flow over a static DrivAer automotive model has been chosen. It had
already been studied in ain similar form as case~2 in the AutoCFD2
workshop~\cite{autocfd2} and as case~2a in the AutoCFD3 and AutoCFD4
workshops~\cite{autocfd3,autocfd4}, so reference results were available tofor
validatevalidating submissions.

The challenge case is the open-closed cooling DrivAer (occDrivAer) configuration: external aerodynamic flow around a full car with closed cooling inlets and static wheels.
The geometry is based on the notchback variant of the Ford Open Cooling DrivAer~(OCDA), with a complex underbody and engine bay cooling channels.
For OHC-1 it was configured as a steady-state, incompressible RANS simulation using the SIMPLE algorithm with fixed inner iterations. Several meshes were pre-generated using snappyHexMesh with three resolutions: 65, 110 and 236 million cells, which were denoted as 65M, 110M and 236M, respectively.
The case is available in the HPCTC repository\footnote{\url{https://develop.openfoam.com/committees/hpc/-/tree/develop/incompressible/simpleFoam/occDrivAerStaticMesh}}.
The $k$--$\omega$ SST turbulence model was employed with pre-defined \texttt{fvSchemes}.
Key case parameters are given in \Cref{tab:case_properties}.
The Reynolds number based on wheelbase $L_\text{ref}$ and inlet velocity is approximately $7.2\times 10^6$.

\begin{table}[!ht]
  \caption{Case properties for the occDrivAer challenge case.}
  \label{tab:case_properties}
  \begin{tabular}{lrc}
    \toprule
    Kinematic viscosity (Air) $\nu$ & $1.507 \cdot 10^{-5}$ & $\mathrm{m}^2/\mathrm{s}$ \\
    Inlet velocity $U$ & $38.889$ & $\mathrm{m}/\mathrm{s}$ \\
    Wheelbase $L_\text{ref}$ & 2.78618 & m \\
    Reynolds number Re & $7.1899\cdot 10^{6}$ & -- \\
    \bottomrule
  \end{tabular}
\end{table}

\Cref{fig:case_geometry} shows the geometry and representative mesh views: the full occDrivAer configuration, a mid-plane section, and an underbody cut.

\begin{figure*}[!ht]
  \centering
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/occDrivAer.png}
    \caption{occDrivAer geometry.}
    \label{fig:occDrivAer}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/mesh_mid_center.png}
    \caption{Mid-plane mesh.}
    \label{fig:mesh_mid}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/mesh_underbody_cut_axle.png}
    \caption{Underbody mesh (cut at axle).}
    \label{fig:mesh_underbody}
  \end{subfigure}
  \caption{Challenge case geometry and mesh.}
  \label{fig:case_geometry}
\end{figure*}


==> parts_refactored/softwaretrack_broken.tex <==
\subsection{Software Track} \label{sec:software_track} \label{sec:res_software_track}

The software track allowed modifications to the default \OF setup to study for example the
impact of solver changes, decomposition strategies, orand hardware-specific
optimisations. While hardware was unconstrained, the mesh and physical modelling
(spatial and temporal discretisation, turbulence model) had to remain
unchanged. Contributions from five organisations (Engys, CINECA, Huawei,
Wikki~GmbH, and KIT/TUM) fell into the following broad categories:
\begin{itemize}
\item Full GPU ports \cite{bna2025spuma} (Engys, CINECA)
\item Offloading of linear solvers to GPUs via OGL \cite{Olenik2025Towards, olenik2025investigating} (KIT/TUM)
\item Decomposition optimisations \cite{popovac_2025} (Wikki, KIT/TUM)
\item Mixed precision \cite{Delorme2024} (Huawei, CINECA)
\item Selective memory allocation \cite{popovac_2025}  (Huawei)
\item Coherent I/O \cite{weiss2024coherent} (Wikki)
\end{itemize}
In the following only a high level overview of the impact of the optimization techniques is presented, a full discussion of the individual techniques is outside the scope of this work and the interested reader is referred to individual publications and conference contributions in \cite{popovac_2025}. 

Because software-track submissions targeted improvements in energy efficiency,
throughput, and time-to-solution, their key metrics were expected to differ from
the hardware-track baseline. 
\Cref{tab:comp-soft-hardw} summarises selected
metrics comparing the best software-track and hardware-track results.
The software track currently represented approximately 26\% of total submissions;
the organisers aim to increase this proportion in future editions.
Because software-track submissions targeted improvements in energy efficiency,
throughput, and time-to-solution, their key metrics were expected to differ from
the hardware-track baseline. 

\begin{table}[!ht]
  \caption{Comparison of best key software-track vs.\ hardware-track metrics.}
  \label{tab:comp-soft-hardw}
  \begin{tabular}{lccc}
    \toprule
    \thead{Metric} & \thead{Software Track} & \thead{Hardware Track} & \thead{Change} \\
    \midrule
    Submitted results & 62 & 175 & 26\% of total \\
    Minimum energy per iteration [J] & 1867 & 2613 & $-28$\% \\
    Maximum performance per node [MFVOPS] & 737 & 629 & $+17$\% \\
    Minimum time per iteration [s] & 0.11 & 0.37 & $-70$\% \\
    \bottomrule
  \end{tabular}
\end{table}

\subsubsection{FVOPS per node and energy per iteration}

\Cref{fig:overview_hardware_vs_software_track} shows FVOPS per node versus
energy per iteration~(J), with hardware-track points in grey and software-track
points coloured by optimisation type. Software-track submissions concentrate in
the upper-left region of the plot, indicating higher throughput and lower energy
per iteration. Full GPU ports and selective-memory optimisations achieved the
highest FVOPS per node, with the best software-track result reaching
approximately 4.2$\times$ the maximum hardware-track performance per node.

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.9\textwidth]{figures/FVOPS_per_Node_EnergyPerIteration_withHWTrack.png}
  \caption{FVOPS per node vs.\ energy per iteration (J). Grey: hardware track;
    coloured: software track by optimisation category.}
  \label{fig:overview_hardware_vs_software_track}
\end{figure}

\subsubsection{Distribution of submissions}

\Cref{fig:relation_hardware_vs_software_track} illustrates the distribution of software-track submissions. \Cref{fig:relation_hardware_vs_software_track_mesh} shows the number of hardware- and software-track submissions across different mesh sizes.
Most software-track data points correspond to the fine mesh, both in absolute numbers and relative to the hardware-track submissions.
The breakdown of optimization categories, shown in \Cref{fig:relation_hardware_vs_software_track}, indicates that the majority of submissions focused on coherent I/O and multilevel decomposition. These are followed by selective memory allocation, mixed-precision solvers, custom decomposition techniques, and full GPU ports.
An analysis of the distribution of the optimization categories across different node counts reveals that several optimization approaches—such as linear solver offloading, full GPU ports, mixed-precision methods, and selective memory allocation, were primarily investigated at smaller scales, up to 16 nodes. In contrast, multilevel decomposition and coherent I/O were also explored at larger scales, exceeding 64 nodes. Custom communication-optimized decomposition strategies were studied in the intermediate range, between 16 and 64 nodes. In addition to the CPU models evaluated in the hardware track, nine submissions utilized GPUs. These included six runs on NVIDIA A100-64, three on NVIDIA A100-40, and one on AMD MI100. It is anticipated that future iterations of the OHC will feature a broader range of GPU models.

%\Cref{fig:relation_hardware_vs_software_track} illustrates the  relative
distribution of the differenthardware- vs.\ software-track submissions.
% by node count and mesh
size\Cref{fig:relation_hardware_vs_software_track_mesh} shows number of hardware and software track submissions for different mesh sizes.
%Most software track datapoints have been submitted for the fine mesh, both in absolute numbers and relative to the hardware-track submissions.
%The break down of the different optimization categories is illustrated in \cref{fig:relation_hardware_vs_software_track}, it can be seen that most submissions concerned coherent IO and multilevel decomposition, followed by selective memory allocation, mixed precission solver, a custom decomposer technology, and full GPU ports.
%The breakdown by category for differen number of compute nodes, shows  that several optimization techniques like linear solver offloading, full GPU ports, mixed-precision, and selective memory allocations were studied rather at smaller node counts up to 16 nodes. In contrast, techniques like multilevel decomposition and coherent IO were investigated also on node counts above 64 nodes. A custom  communication optimization decomposition was investigated in the range of 16 till 64 nodes.
. %Software-track submissions are relatively more numerous at larger node 
counts and on the fine mesh, which partly explains the spread in energy per 
iteration (communication overhead and mesh size both affect energy consumption).
The software track currently represented approximately 26\% of total submissions;
the organisers aim to increase this proportion in future editions.

\begin{figure}[!ht]
  \centering
    \begin{subfigure}[b][5cm][]{0.20\textwidth}
    \includegraphics[height=4.5cm]{figures/Count_Mesh_Track.png}
    \caption{Distribution by node count.\label{fig:relation_hardware_vs_software_track_mesh}}
  \end{subfigure}
  \hfill
    \begin{subfigure}[b][5cm][]{0.70\textwidth}
    \includegraphics[height=4.5cm]{figures/Count_Nodes_Category.png}
    \caption{Distribution by mesh and nodes.}
  \end{subfigure}
  \caption{DRelative distribution of hardware- vs.\ software-track submissions, (a) distribution of hardware and software track contributions by mesh type, (b) Distribution of software optimization category contributions over number of nodes.}
  \label{fig:relation_hardware_vs_software_track}
\end{figure}

\subsubsection{FVOPS per node and energy per iteration}
\Cref{fig:overview_hardware_vs_software_track} shows measured FVOPS per node versus
energy per iteration in Joule for all submissions, with  software-track
points coloured by optimisation type and
hardware-track points in grey as reference. Since most submissions investigated strong scaling behaviour data points tend to cluster along diagonal lines since the required energy per iteration increases with increasing number of compute nodes, due to increasing communication overhead. Several 
Software-track data points can be found in
the upper-left region of the plot, indicating higher throughput per node and a lower energy
consumption per iteration compared to the default \OF version. Here, namely the selective memory allocation optimization reduced the minimum required electric energy from 2613 Joule to 1867 Joule per iteration. Additionally, full GPU ports and selective-memory optimisations achieved the highest FVOPS per node, with 58 and 36 MFVOPS respectively, with the best software-track result reaching
approximately 4 $\times$ the maximum hardware-track performance of 14 MFVOPS per node. 
\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.75\textwidth]{figures/FVOPS_per_Node_EnergyPerIteration_withHWTrack.png}
  \caption{FVOPS per node vs.\ energy per iteration in Joules. Grey: hardware track;
    coloured: software track by optimisation category.}
  \label{fig:overview_hardware_vs_software_track}
\end{figure}
The increased peak performance is further reflected in the reported minimum wall-clock time required to compute a single timestep. As shown in \cref{tab:minimum_timestep}, the largest improvements are observed for the coarsest mesh, with a reduction of 72\%, followed by the medium mesh, which exhibits a reduction of 44\%.

\begin{table}[!h]
\caption{Reported minimum time per timestep.\label{tab:minimum_timestep}}
\begin{tabular}{l | lll} \toprule
  Mesh & coarse & medium & fine \\    \midrule 
Hardware Track    &  0.42  &   0.65     &   0.37   \\
Software Track    &  0.11  &   0.36     &   0.32   \\ \midrule
Change       &   -72 \%   & -44 \%  &  -14\%        \\ \bottomrule
\end{tabular}
\end{table}

It is important to note that, although full GPU ports exhibited the highest per-node performance, their comparatively limited strong-scaling efficiency constrained their overall performance. Consequently, alternative optimization strategies, such as custom decomposition approaches and coherent I/O achieved the highest aggregate performance in terms of FVOPS. This behavior is illustrated in \cref{fig:sw_fvops_nodes_gpu}, which depicts FVOPS as a function of the number of compute nodes for the fine mesh, categorized by optimization strategy.
Nevertheless, GPU-based implementations required substantially fewer compute nodes to achieve comparable peak performance relative to CPU-only optimization approaches, corresponding to a reduction of approximately one order of magnitude (i.e., a factor of 10–15). 

%Addtionally, the increase of the peak performance 

%\Cref{fig:sw_fvops_nodes_gpu} shows FVOPS versus node count for all
%software-track submissions, classified by GPU type (full GPU port, GPU plugin, or
%other/CPU-only) and distinguished by GPU model. Full GPU port submissions (Engys
%and CINECA) achieve the highest absolute FVOPS, followed by GPU plugin
%submissions (KIT/TUM). 

%CPU-only software optimisations (decomposition, mixed precision, selective memory, coherent I/O) achieve lower absolute throughput but, as shown in the preceding figures, can still significantly outperform the hardware-track baseline per node.

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.75\textwidth]{figures/FVOPS_Nodes_GPUOptimizationType_Fine_fit.png}
  \caption{FVOPS vs.\ node count for software-track submissions, coloured by optimization category. Trendlines using polynomial regression are shown as colored dashed lines. }
  \label{fig:sw_fvops_nodes_gpu}
\end{figure}

\iffalse
\subsubsection{FVOPS vs.\ energy by optimisation category}

\Cref{fig:sw_fvops_energy_optcat} provides an alternative view of throughput
versus energy efficiency, with software-track submissions coloured by their
declared optimisation category. Categories with higher FVOPS and lower energy per
iteration (upper-left region) represent the most effective optimisations.
Submissions labelled as decomposition-focused and selective-memory optimisations
occupy favourable positions, demonstrating that CPU-level software improvements
can be highly competitive with GPU-based approaches in terms of energy efficiency.
\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.95\textwidth]{figures/sw_FVOPS_Energy_OptCat.png}
  \caption{FVOPS vs.\ energy per iteration (J) for software-track submissions,
    coloured by optimisation category.}
  \label{fig:sw_fvops_energy_optcat}
\end{figure}
\fi
\subsubsection{FVOPS by GPU type and node count}

\Cref{fig:sw_fvops_nodes_gpu} shows FVOPS versus node count for all
software-track submissions, classified by GPU type (full GPU port, GPU plugin, or
other/CPU-only) and distinguished by GPU model. Full GPU port submissions (Engys
and CINECA) achieve the highest absolute FVOPS, followed by GPU plugin
submissions (KIT/TUM). CPU-only software optimisations (decomposition, mixed
precision, selective memory, coherent I/O) achieve lower absolute throughput but,
as shown in the preceding figures, can still significantly outperform the
hardware-track baseline per node.

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.95\textwidth]{figures/sw_FVOPS_Nodes_GPUType.png}
  \caption{FVOPS vs.\ node count for software-track submissions, coloured by GPU
    acceleration type and styled by GPU model.}
  \label{fig:sw_fvops_nodes_gpu}
\end{figure}

\subsubsection{FVOPS vs.\ energy by optimisation category}

\Cref{fig:sw_fvops_energy_optcat} provides an alternative view of throughput
versus energy efficiency, with software-track submissions coloured by their
declared optimisation category. Categories with higher FVOPS and lower energy per
iteration (upper-left region) represent the most effective optimisations.
Submissions labelled as decomposition-focused and selective-memory optimisations
occupy favourable positions, demonstrating that CPU-level software improvements
can be highly competitive with GPU-based approaches in terms of energy efficiency.

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.95\textwidth]{figures/sw_FVOPS_Energy_OptCat.png}
  \caption{FVOPS vs.\ energy per iteration (J) for software-track submissions,
    coloured by optimisation category.}
  \label{fig:sw_fvops_energy_optcat}
\end{figure}
\iffalse
\subsubsection{FVOPS by GPU type and node count}
\subsubsection{Fine mesh: software vs.\ hardware track comparison}

\Cref{fig:sw_fvops_energy_fine_hw} isolates the fine mesh (236\,M cells), which
is the most computationally demanding and industrially relevant configuration.
Hardware-track submissions are shown in grey; software-track submissions are
coloured by optimisation category. On the fine mesh, the performance gap between
software-track and hardware-track submissions is particularly pronounced: GPU
ports achieve FVOPS values that are several times higher than the best CPU-only
hardware-track runs, while also consuming less energy per iteration. This
confirms that the fine mesh provides the clearest signal for evaluating software
optimisations, and future OHC editions should encourage participants to focus on
this mesh size.

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.95\textwidth]{figures/sw_FVOPS_Energy_fine_vs_HW.png}
  \caption{Fine mesh only: FVOPS vs.\ energy per iteration (J).  Grey
    markers: hardware track; coloured markers: software track by
    optimisation category.}
  \label{fig:sw_fvops_energy_fine_hw}
\end{figure}

\subsubsection{Scaling of energy and time per iteration}

\Cref{fig:sw_energy_time_cores} shows energy per iteration (left) and time per
iteration (right) as a function of CPU core count, with markers distinguished by
GPU model and mesh size. Several trends are apparent:
\begin{itemize}
\item GPU-accelerated submissions (A100, on-package/HBM) achieve the lowest time
  per iteration at comparable or lower energy cost.
\item Energy per iteration generally increases with core count, reflecting
  communication and idle-core overhead at scale.
\item Time per iteration decreases with core count, but with diminishing returns
  at high core counts---consistent with the strong-scaling limits observed in the
  hardware track.
\item The fine mesh is more sensitive to both energy and time scaling than the
  coarse or medium meshes, reinforcing the importance of testing at industrially
  relevant scales.
\end{itemize}


\begin{figure*}[!ht]
  \centering
  \includegraphics[width=0.95\textwidth]{figures/sw_energy_time_per_iter_cores.png}
  \caption{Software track: energy per iteration (left) and time per iteration
    (right) vs.\ number of CPU cores.  Coloured by GPU model, styled by mesh
    size.}
  \label{fig:sw_energy_time_cores}
\end{figure*}
\fi
\subsubsection{Aerodynamic coefficient consistency}

An important quality metric for software-track submissions is the consistency of
the computed aerodynamic force coefficients across different optimisation
approaches and hardware. \Cref{fig:sw_aero_boxplot} shows box-and-strip plots of
the mean drag ($C_d$), lift ($C_l$), and side-force ($C_s$) coefficients across
all submissions (excluding one outlier contributor). The narrow interquartile
ranges for $C_d$ and $C_s$ indicate that most optimisations preserve solution
accuracy well. The slightly wider spread for $C_l$ reflects the known sensitivity
of lift to solver settings, turbulence-model numerics, and convergence criteria.
Overall, the distributions confirm that software-track submissions maintained
acceptable agreement with the reference values, validating the meanCalc-based
quality checking procedure described in \Cref{sec:validation}.

\begin{figure*}[!ht]
  \centering
  \includegraphics[width=0.85\textwidth]{figures/sw_aero_coefficients_boxplot.png}
  \caption{Distribution of mean aerodynamic force coefficients ($C_d$, $C_l$,
    $C_s$) across all submissions.  Box plots show medians and interquartile
    ranges; individual submissions are overlaid as strip points.}
  \label{fig:sw_aero_boxplot}
\end{figure*}

